Killip-Simon-classes of Jacobi matrices with essential spectrum on two symmetric and of SMP matrices on two arbitrary intervals

Jacobi matrices probably are the most classical object in spectral theory, while CMV matrices are a comparably fresh one, although they are related to a very classical topic, namely to orhtogonal polynomials on the unit circle (in the same way as Jacobi matrices are related to orhogonal polynomials on the real axis). We will discuss the third member of this family. Our matrices are generated by the orthonormal systems of functions related to the so-called Strong Moment Problem. For this reason we call them SMP matrices. For instance, one can describe the spectral sets of periodic SMP matrices. Similarly to the case of their counterparts, the description is given by means of conformal mappings on hyperbolic, in this case, comb domains. One can represent functional models associated with periodic and almost periodic SMP matrices. We are especially enthusiastic about the role, which such matrices can play in the Killip-Simon-problem related to Jacobi matrices with the essential spectrum on two arbitrary intervals. The parametric description of SMP matrices of the Killip-Simon-class with their essential spectrum on two arbitrary intervals is the main result of this paper.

==> 0.1jintro.tex <==
In this section we consider a real measure $\sigma$, whose support we assume to be compact. By applying the Gram-Schmidt orthogonalization
procedure to the family of polynomials $\{x^n\}_{n\geq0}$ w.r.t. $\ud\sigma$, we obtain orthonormal polynomials
$P_n=\alpha_{n}^{(n)}x^n+\cdots+\alpha_{0}^{(n)}$, where $\alpha_n^{(n)}>0$. It is a well-known fact that these polynomials obey
the following three-term recurrence
\begin{equation*}
 z P_n=a_{n+1}P_{n+1}+b_{n}P_{n}+a_{n}P_{n-1},
\end{equation*}
with $a_n$ positive and
where we set $P_{-1}\equiv0$.

The corresponding three-diagonal Jacobi matrix we denote by $J_+$, that is
\begin{equation*}
 J_+=S_+\ba_+ +\bb_+ +\ba_+ S_+^*,
\end{equation*}
where $\{a_n\}_{n\geq1}$ and $\{b_n\}_{n\geq0}$ are two bounded real sequences such that $a_n>0$. Furthermore,
 $\mathcal A_+=\diag\{a_n\}$ and  $\mathcal B_+=\diag\{b_n\}$ and $S_+$ denotes the shift operator on the positive half axis.
Recall that any Jacobi matrix, which defines a bounded self-adjoint operator in $\ell^2_+$, can be obtained in this way.

In the next section we will consider periodic Jacobi matrices. Such matrices possess a natural extension to the negative half axis.
That is, we will also consider two-sided Jacobi matrices.


Given two bounded real sequences $\{a_n\}_{n\in\mathbb Z}$, $a_n>0$, and $\{b_n\}_{n\in\mathbb Z}$ we define a two-sided Jacobi matrix
by
\begin{equation*}
 J=S\ba +\bb +\ba S^{-1},
\end{equation*}
where $\ba$ (resp. $\bb$) is a two-sided diagonal matrix, whose entries are the elements of the sequence $\{a_n\}$ (resp. $\{b_n\}$)
and where $S$ denotes the two-sided shift operator acting on the entire $\ell^2$.



==> 1.1jisospectral.tex <==
In this section we are going to discuss two-periodic Jacobi matrices whose essential spectrum is composed of two disjoint intervals
of equal length. To this end we introduce  $\tilde E$ as the union of these intervals. To any such $\tilde E$ there corresponds a 
quadratic polynomial $\tilde T(z)$ such that 
  $\tilde E=\tilde T^{-1}\left([-2,2]\right)$. Through a linear change of variables, however, we may as well consider
\begin{equation*}
 T(z)=z^2-\lambda,\quad \lambda>2
\end{equation*}
and $E=T^{-1}([-2,2])$.


Also, if we have an arbitrary two-sided Jacobi matrix of period two
\begin{equation*}
\label{eqn:jtilde}
 \tilde J =
  \begin{pmatrix}
   \ddots	&	\ddots	&	\ddots	\\
		&	a_0	&	b_0	&	a_1	\\
		&		&	a_1	&	b_1	&	a_0	\\
		&		&		&	a_0	&	b_0	&	a_1	\\
		&		&		&		&	a_1	&	b_1	&	a_0	\\
		&		&		&		&		&	\ddots	&	\ddots	&	\ddots
  \end{pmatrix},
\end{equation*}
where $a_i>0$ and $b_i\in\mathbb R$, $i\in\{0,1\}$, then there exist constants $\tilde a$ and $\tilde b$ such that
\begin{equation*}
 J_0\deq \tilde a \tilde J+\tilde b=\begin{pmatrix}
   \ddots	&	\ddots	&	\ddots	\\
		&	a	&	b	&	\frac{1}{a}	\\
		&		&	\frac{1}{a}	&	-b	&	a	\\
		&		&		&	a	&	b	&	\frac{1}{a}	\\
		&		&		&		&	\frac{1}{a}	&	-b	&	a	\\
		&		&		&		&		&	\ddots	&	\ddots	&	\ddots
  \end{pmatrix}.
\end{equation*}
for some $a>0$ and $b\in\mathbb R$.

In what follows, let us denote by $J_0(E)$ the set of all period-2 Jacobi matrices $J_0$ of the above form such that the 
spectrum of $J_0$ is given by $E$, or, equivalently, such that $T(J_0)=S^2+S^{-2}$.


\begin{thmjiso}
 \label{thm:jiso}
For $\lambda>2$ we have that
\begin{equation*}
 J_0\in J_0(E) \quad\Longleftrightarrow\quad u^2+b^2=r^2,
\end{equation*}
where $u=a-a^{-1}$ and $r=\sqrt{\lambda-2}$.
\end{thmjiso}
\begin{proof}
 From $J_0^2-\lambda=S^2+S^{-2}$ we immediately obtain
\begin{equation*}
 0=a^2+\frac{1}{a^2}+b^2-\lambda=\left(a-\frac{1}{a}\right)^2+b^2-(\lambda-2).
\end{equation*}
\end{proof}
Hence, the isospectral equation describes a circle in the $(u,b)$-plane.


==> 1.2jksclass.tex <==
\begin{defjks}
 \label{def:jks}
A two-sided matrix $A$ is in the \emph{Hilbert-Schmidt-class} ($A\in\hs$) if $\tr(A^*A)<\infty$, where, as usual for positive
matrices, the trace $\tr(\cdot)$ can be defined as a series of diagonal elements.
 Moreover,  we say that a Jacobi matrix $J$ is in the \emph{Killip-Simon-class}
($J\in\ks_J(E)$) if $T(J)-\left(S^2+S^{-2}\right)$ is of the Hilbert-Schmidt class.
\end{defjks}

This class was originally discovered and studied in \cite{refjreview}. For recent progress in the understanding of finite
gap Jacobi matrices and their pertubations see \cite{jreview}.

In what follows, we give an explicit parametric description  of Jacobi matrices which belong to the Killip-Simon-class. 
To this end, let from now
on $\lambda>2$ and let $J$ be an arbitrary, two-sided Jacobi matrix. The following result immediately follows from the above definition.

\begin{lemmajoriginalcond}
 \label{lemma:joriginalcond}
 $J$ is in the Killip-Simon-class if and only if the following conditions are fulfilled:
\begin{align}
 \tag{J1}
 a_{n}a_{n+1}-1 &\in\ell^2	 \label{eqn:J1}\\
 \tag{J2}
a_{n+1}\left(b_n+b_{n+1}\right)&\in\ell^2.	 \label{eqn:J2}\\
 \tag{J3} 
a_{n}^2+a_{n+1}^2+b_{n}^2-\lambda &\in\ell^2.	 \label{eqn:J3}
\end{align}
\end{lemmajoriginalcond}

\begin{rempub}
 \label{rem:pub}
Note that, due to condition (\ref{eqn:J3}), we have that
\begin{equation*}
 \frac{4}{\lambda+1}<a_n^2<\lambda+1
\end{equation*}
and as $a_n>0$ we get that $\{\log a_n\}$ is uniformly bounded.
\end{rempub}

\begin{lemmajprimecond}
 \label{lemma:jprimecond}
The set of conditions (\ref{eqn:J1}), (\ref{eqn:J2}), (\ref{eqn:J3}) is equivalent to
\begin{align}
   \tag{J1'}
 u_{n}+u_{n+1} &\in\ell^2,	 \label{eqn:J1p}\\
  \tag{J2'}
b_n+b_{n+1}&\in\ell^2,	 \label{eqn:J2p}\\
  \tag{J3'} 
u_{n}^2+b_{n}^2-r^2&\in\ell^2,	 \label{eqn:J3p}
\end{align}
where $u_n=a_n-a_n^{-1}$ and $r=\sqrt{\lambda-2}$.
\end{lemmajprimecond}
\begin{proof}
 For (\ref{eqn:J1p}) we obtain
\begin{equation*}
 u_n+u_{n+1}=a_n-\frac{1}{a_n}+a_{n+1}-\frac{1}{a_{n+1}}=\left(a_na_{n+1}-1\right)\left(\frac{1}{a_n}+\frac{1}{a_{n+1}}\right).
\end{equation*}
Due to Remark~\ref{rem:pub} the last factor is uniformly bounded and hence this is equivalent to (\ref{eqn:J1}). Also
because of the uniform boundedness of $\{\log a_n\}$ we see that $(\ref{eqn:J2})\Leftrightarrow(\ref{eqn:J2p})$. For the proof
of the last equivalence we first observe that
\begin{equation*}
a_n^2+a_{n+1}^2 = \frac{1}{a^2_n}\left(a_n^2a_{n+1}^2-1\right) + a_{n}^2+\frac{1}{a^2_n}.
\end{equation*}
Note that $a_n^2a_{n+1}^2-1\in\ell^2$ iff $a_na_{n+1}-1\in\ell^2$, which is (\ref{eqn:J1}). Thus,
\begin{equation*}
 (\ref{eqn:J3})\Leftrightarrow  a_{n}^2+\frac{1}{a^2_n}+b_n^2-\lambda\in\ell^2\Leftrightarrow
\left( a_{n}-\frac{1}{a_n}\right)^2+b_n^2-(\lambda-2)\in\ell^2
\end{equation*}
\end{proof}

We now rewrite our parameters $u_n$ and $q_n$ by means of polar coordinates, i.e.
\begin{equation*}
 u_n=r_n\cos\phi_n\qquad\text{and}\qquad b_n=r_n\sin\phi_n.
\end{equation*}
This allows us to state the main theorem of this section.
\begin{thmjkscond}
 \label{thm:jkscond}
Let $\lambda>2$ and let $J$ be a two-sided Jacobi matrix. Then, $J\in\ks_J(E)$ if and only if there exist two $\ell^2$-sequences
$\{\alpha_n\}$, $\{\beta_n\}$ such that
\begin{align*}
 r_n &=\sqrt{\lambda-2}+\alpha_n\quad \text{and}\\
 \phi_n &= \pi n+\sum_{k=0}^{n}\beta_k,
\end{align*}
where
\begin{align*}
 a_n-\frac{1}{a_n} &= r_n\cos\phi_n\quad\text{and}\\
 b_n&=r_n\sin\phi_n.
\end{align*}
\end{thmjkscond}
\begin{proof}
 Obviously,
\begin{equation*}
 (\ref{eqn:J3p})\Leftrightarrow r_n^2-r^2\in\ell^2\Leftrightarrow r_n-r=\alpha_n\in\ell^2,
\end{equation*}
Considering this in (\ref{eqn:J1p}) and in (\ref{eqn:J2p}) we get that
\begin{equation*}
 \cos\phi_n+\cos\phi_{n+1}\in\ell^2\quad \text{and} \quad \sin\phi_n+\sin_{n+1}\in\ell^2.
\end{equation*}
Rewriting the cosines and sines by means of exponential functions and adding the above conditions yields
\begin{align*}
 (\ref{eqn:J1p}),(\ref{eqn:J2p}) &\Leftrightarrow e^{\im\phi_{n+1}}+e^{\im\phi_n}\in\ell^2
\Leftrightarrow \cos\left(\frac{\phi_{n+1}-\phi_n}{2}\right)\in\ell^2\\
&\Leftrightarrow \sin\left(\frac{\phi_{n+1}-\phi_n}{2}-\frac{\pi}{2}\right)\in\ell^2\\
&\Leftrightarrow \phi_{n+1}-\phi_{n}-\pi=\beta_n \in\ell^2.
\end{align*}

\end{proof}


==> 1.Introduction.tex <==
Suppose we are given a compactly supported real measure $\sigma$ whose support does not contain zero and consider the linearly 
independent family of functions
\begin{equation*}
 1,~\frac{-1}{z},~z,~\left(\frac{-1}{z}\right)^2,~z^2,~,\ldots
\end{equation*}
Subsequently, we orthogonalize these functions with respect to $\ud\sigma$, giving
\begin{equation*}
 \tilde \Psi_0 = 1,\qquad
 \tilde \Psi_{2n-1}=\left(\frac{-1}{z}\right)^n+\alpha_1z^{n-1}+\cdots,\qquad
 \tilde \Psi_{2n}=z^n+\beta_1\left(\frac{-1}{z}\right)^{n}+\cdots,
\end{equation*}
and normalize them by setting
\begin{equation}
\label{eqn:normalize}
 \Psi_n= \frac{\tilde \Psi_n}{\|\tilde \Psi_n\|}.
\end{equation}
We denote this family by $\boldsymbol \Psi=\{\Psi_n\}_{n\in\mathbb N_0}$. Note that 
$\boldsymbol \Psi$ forms a complete orthonormal system in $L^2(\ud\sigma)$. This system of orthonormal rational functions is also considered
in \cite[(2.2) and (2.3)]{shmp} and for more general orthogonal systems of rational functions see  \cite{schur}.

\begin{lemmarecursion}
 \label{lemma:recursion}
Using the same notation as in the above paragraphs we have
\begin{IEEEeqnarray*}{c c ccccccccc}
z\Psi_{m} &=& r_{m} \Psi_{m-2}&+&p_{m}\Psi_{m-1}&+&q_{m}\Psi_{m}&+&p_{m+1}\Psi_{m+1}&+&r_{m+2}\Psi_{m+2},\\ 
\frac{1}{z} \Psi_{m} &=& \rho_{m}\Psi_{m-2}&+&\pi_{m}\Psi_{m-1}&+&\sigma_{m}\Psi_{m}&+&\pi_{m+1}\Psi_{m+1}&+&
\rho_{m+2}\Psi_{m+2},
\end{IEEEeqnarray*}
where $p_m, q_{m},r_m,\pi_m,\sigma_m$ and $\rho_{m}$ denote some coefficient sequences. Moreover, $r_{2n}>0,~ r_{2n+1}=0$ and
$\rho_{2n}=0,~ \rho_{2n+1}<0$.
\end{lemmarecursion}


We now pass from square integrable functions w.r.t. $\mathrm d \sigma$  to the one-sided sequence space $\ell^2_+$.
To this end we define 
$A_+$ as the matrix of the multiplication operator by $z$ and $A_+^{-1}$ is the matrix of the multiplication operator by
$z^{-1}$. We refer to $A_+$ as \emph{one-sided SMP matrix}. As a direct consequence of Lemma~\ref{lemma:recursion} we obtain
the following theorem.

\begin{thmstructureonesided}
\label{thm:structureonesided}
We have that
\begin{equation*}
 A_+=S^2_+ \br_+ + S_+ \bp_+ + \bq_+ + \bp_+ S_+^* + \br_+ (S_+^{*})^2 ,
\end{equation*}
where, for $n\geq0$, $\bp_+ = \diag\{p_n\}$, $\bq_+ = \diag\{q_n\}$ as well as
 $\br_+$ $= \diag\{r_{n}\}$ are one-sided diagonal matrices and where  $r_{2n}>0,~r_{2n+1}=0$.
Moreover,
\begin{equation*}
A_+^{-1}= S_+^2 \mathbf P_+ + S_+\mathbf \Pi_+ + \mathbf \Sigma_+ + \mathbf \Pi_+ S_+^{*} + \mathbf P_+ (S_+^{*})^2,
\end{equation*}
 where $\mathbf P_+ = \diag\{\rho_{n}\}$, $\mathbf \Sigma_+ = \diag\{\sigma_n\}$ and 
$\mathbf \Pi_+$  $= \diag\{\pi_n\}$ and where $\rho_{2n+1}<0,~\rho_{2n}=0$.
\end{thmstructureonesided}


\begin{remstructureonsided}
 \label{rem:structureonesided}
Note that $A_+$ possesses the same structure as its shifted inverse equipped with a negative sign.
Also, since $A_+ A_+^{-1}=\id$ there exist several algebraic relations between the entries of $A_+$ and $A_+^{-1}$.
\end{remstructureonsided}



==> 3.isospectral.tex <==
Suppose we are given two disjoint intervals, whose union we denote by $\tilde E$. Then we can always find a function
\begin{equation*}
 \tilde V(z)=a z+b+\frac{\varrho}{c-z},\quad a>0,\ \varrho>0,
\end{equation*}
such that
\begin{equation*}
 \tilde E =\tilde V^{-1}\left([-2,2]\right)=\left\{z\!:~\tilde V(z)\in[-2,2]\right\}.
\end{equation*}
By a linear change of variables we can reduce $\tilde V$ such that it suffices to consider
\begin{equation}
\label{eqn:V}
 V(z)\deq a z+b-\frac{1}{z},
\end{equation}
where $a>0$ and $b\in\mathbb R$. Thus, in what follows $E$ is assumed to be the preimage of $V$ of $[-2,2]$, i.e.
\begin{equation*}
 E\deq\left\{z\!: a z+b-\frac{1}{z}\in[-2,2]\right\}.
\end{equation*}
$E$ constitutes the union of two arbitrary intervals about zero, see Fig.~1, whose
end points are given by 

\begin{IEEEeqnarray*}{rllrll}
\phantomsection
\label{eqn:gaps}
b_0 &= -&\sqrt{\left(\frac{b+2}{2a}\right)^2+\frac{1}{a}}-\frac{b+2}{2a},~
&a_1 &= -& \sqrt{\left(\frac{b-2}{2a}\right)^2+\frac{1}{a}}-\frac{b-2}{2a},\IEEEyesnumber\\ 
b_1 &=&  \sqrt{\left(\frac{b+2}{2a}\right)^2+\frac{1}{a}}-\frac{b+2}{2a},~
&a_0 &=& \sqrt{\left(\frac{b-2}{2a}\right)^2+\frac{1}{a}}-\frac{b-2}{2a}.
\end{IEEEeqnarray*}

\begin{figure}[!hbtp]
\phantomsection
\label{fig:e}
 \centering
  \includegraphics[width=0.6\textwidth]{e.jpg}
 \caption[Exemplary Plot of $E$]{Exemplary plot of $E$ for $a=2.5$ and $b=-3$.}
\end{figure}

\begin{defisotorus}
 \label{def:isotorus}
By $A_0(E)$ we denote the set of all SMP matrices of period two with their spectrum on  $E$.
\end{defisotorus}


\begin{thmisospectral}
 \label{thm:isospectral}
 Let $a>0$, $b\in\mathbb R$ and let $V$ and $E$ be given as above. Then the following three statements are equivalent:
\begin{align}
\tag{i}A_0\in A_0(E),\\
 \tag{ii} V(A_0)=S^2+S^{-2}, \\
\tag{iii} r_1=r=\frac{1}{a},\ q_0+q_1=-\frac{b}{a} \text{ and}\\
\label{eqn:isospectral} p_0^2+p_1^2+a^2p_0^2p_1^2+bp_0p_1 =\frac{1}{a},
\end{align}
\end{thmisospectral}

\begin{proof}
 From the identity $V(A_0)=S^2 + S^{-2}$ we can derive the following system of equations:
\begin{align}
 \tag{i}
ar &= 1	\label{eqn:i}\\
\tag{ii}
-\rho_0=-\rho&=1		\label{eqn:ii}\\
\tag{iii}
ap_0-\pi_0&=0	\label{eqn:iii}\\
\tag{iv}
ap_1-\pi_1&=0	\label{eqn:iv}\\
\tag{v}
aq_0+b-\sigma_0&=0	\label{eqn:v}\\
\tag{vi}
aq_1+b-\sigma_1&=0.	\label{eqn:vi}
\end{align}

The first two items obviously imply that $r=a^{-1}$ and $\rho=-1$. Also, we immediately see that, due to
Theorem~\ref{thm:freeparameters},  (\ref{eqn:iii}) and (\ref{eqn:iv}) are automatically fulfilled. We use (\ref{eqn:vi}) to find that
\begin{equation*}
 q_1=\frac{1}{a}\left(\sigma_1-b\right)=-ap_0p_1-\frac{b}{a},
\end{equation*}
which, in turn, renders (\ref{eqn:v}) obsolete. The only equation that we have not yet fully exploited is the second one.
We have
\begin{IEEEeqnarray*}{LrCl}
& p_0^2r+p_1^2r -q_1 p_0p_1 &=& r^2\\
\Longleftrightarrow \quad&  p_0^2+p_1^2+a^2p_0^2p_1^2+bp_0p_1 &=& \frac{1}{a}
\end{IEEEeqnarray*}
\end{proof}
% \left(p_0+p_1\right)^2 + \left(ap_0p_1+\frac{b-2}{2a}\right)^2 &=& \frac{1}{a} + \left(\frac{b-2}{2a}\right)^2.

Let us rewrite the isospectral equation (\ref{eqn:isospectral}) in the following way
\begin{equation*}
 \left(p_0+p_1\right)^2 + \left(ap_0p_1+\frac{b-2}{2a}\right)^2 = \frac{1}{a} + \left(\frac{b-2}{2a}\right)^2.
\end{equation*}
If we use the identities from (\ref{eqn:gaps})
 and put $u=p_0+p_1$ and $v=ap_0p_1$, then we obtain
\begin{equation*}
 u^2+\left(v-\frac{a_0+a_1}{2}\right)^2=\left(\frac{a_0-a_1}{2}\right)^2.
\end{equation*}
Note that the critical points of the mapping $(p_0,p_1)\mapsto(u,v)$ correspond to $p_0=p_1=p$ on this curve, see Fig.~3.  From
\begin{equation*}
 a^2p^4+(b+2)p^2-\frac{1}{a}=0
\end{equation*}
we see that these are given by
\begin{IEEEeqnarray*}{rCl}
 \pm u_c&=&\pm2p=\pm \left(
\frac{4}{a} \left(\sqrt{\left(\frac{b+2}{2a}\right)^2+\frac{1}{a}}-\frac{b+2}{2a} \right)
\right)^{\frac{1}{2}}\\
&=&\pm\sqrt{b_1\left(a_0+a_1-b_1-b_0\right)}
\end{IEEEeqnarray*}
and
\begin{equation*}
 v_c=ap^2=\sqrt{\left(\frac{b+2}{2a}\right)^2+\frac{1}{a}}-\frac{b+2}{2a} =b_1.
\end{equation*}
Thus, what is obtained in the $(u,v)$-plane, as a matter of fact, is a part of a circle centered at 
$(0,c)$, $c=(a_1+a_0)/2$, with radius $(a_0-a_1)/2$ and end points $(\pm u_c,v_c)$. Figure~2 shows an exemplary plot
of the isospectral equation in the $(u,v)$-plane.

\begin{figure}[!hbtp]
\phantomsection
\label{fig:iso}
 \centering
 \includegraphics[width=0.5\textwidth]{iso.jpg}
 \caption[Exemplary Plot of the Isospectral Equation]{Exemplary plot of the isospectral equation in the $(u,v)$-plane for $a=2.5$ and $b=-3$.}
\end{figure}


==> 4.ksclass.tex <==
\begin{defks}
 \label{def:ks}
We say that an SMP matrix $A$ is in the \emph{Killip-Simon-class}, or, in short, $A\in\ks_{\smp}(E)$ if and only if
\begin{equation}
 \label{eqn:ks}
 V(A)-\left(S^2+S^{-2}\right)\in\hs,
\end{equation}
where $V$ is defined in (\ref{eqn:V}).
\end{defks}

The following lemma describes when an SMP matrix belongs to the Killip-Simon-class in terms of the parameters 
$p_{2n},p_{2n+1}, q_{2n+1}, r_{2n+1}$.

\begin{lemmaks}
 \label{lemma:ks}
Let $A$ be an SMP matrix. Then,
$A\in\ks_{\smp}(E)$
if and only if the coefficient sequences satisfy the following conditions:
\begin{align}
 \tag{C1}
 r_{2n+1}-\frac{1}{a} &\in\ell^2.	 \label{eqn:C1}\\
 \tag{C2}
 p_n-p_{n-2} &\in\ell^2.	 \label{eqn:C2}\\
 \tag{C3} 
q_{2n+1}+\frac{b}{a}+ap_{2n}p_{2n+1}&\in\ell^2.	 \label{eqn:C3}\\
\tag{C4}
p_{2n}^2+p_{2n+1}^2+a^2p_{2n}^2p_{2n+1}^2+bp_{2n}p_{2n+1}-\frac{1}{a}
&\in\ell^2.	 \label{eqn:C4}
\end{align}
\end{lemmaks}

\begin{proof}
From (\ref{eqn:ks}) we immediately get the conditions
\begin{align}
\tag{c1}
r_{2n+1}-\frac{1}{a} &\in\ell^2,	\label{eqn:c1}\\
\tag{c2}
 \rho_{2n}+1 &\in\ell^2,	\label{eqn:c2}\\
\tag{c3}
 ap_{2n}-\pi_{2n} &\in\ell^2,	\label{eqn:c3}\\
\tag{c4}
ap_{2n+1}-\pi_{2n+1}&\in\ell^2, \label{eqn:c4}\\
\tag{c5}
aq_{2n}+b-\sigma_{2n}&\in\ell^2  \text{ and} \label{eqn:c5}\\
\tag{c6}
aq_{2n+1}+b-\sigma_{2n+1} &\in\ell^2, \label{eqn:c6}
\end{align}
so (\ref{eqn:C1}) is already obtained. Furthermore, it follows from Theorem~\ref{thm:freeparameters} together with the fact
that the sequences $\{\log r_{2n+1}\}$ and $\{p_{n}\}$ are uniformly bounded that
\begin{equation*}
 (\text{\ref{eqn:c3}}) \Leftrightarrow ap_{2n}r_{2n-1}+p_{2n-2}\rho_{2n}\in\ell^2
 \overset{(\text{\ref{eqn:c1}), (\ref{eqn:c2})}}{\Leftrightarrow}
 p_{2n}-p_{2n-2}\in\ell^2.
\end{equation*}
In the same way we can deduce $p_{2n+1}-p_{2n-1}\in\ell^2$ from (\ref{eqn:c4}) and thus obtain (\ref{eqn:C2}).

For the simplification of (\ref{eqn:c6}) we once again use the fact that $r_{2n+1}>0$ uniformly and that $\{p_{n}\}$ is a uniformly 
bounded sequence as well as the identities given in Theorem~\ref{thm:freeparameters}:
\begin{IEEEeqnarray*}{rCl}
 (\text{\ref{eqn:c6}})& \Leftrightarrow& aq_{2n+1}+b-\frac{p_{2n}p_{2n+3}\rho_{2n+2}}{r_{2n+1}r_{2n+3}}\in\ell^2\\
&\overset{\text{(\ref{eqn:c1}), (\ref{eqn:c2})}}{\Leftrightarrow}&
q_{2n+1}+\frac{b}{a}+ap_{2n}p_{2n+3}\in\ell^2\\
&\overset{\text{(\ref{eqn:C2})}}{\Leftrightarrow}&
q_{2n+1}+\frac{b}{a}+ap_{2n}p_{2n+1}\in\ell^2\\
& \Leftrightarrow &(\text{\ref{eqn:C3}}).
\end{IEEEeqnarray*}
For more or less the same reasons we can reduce (\ref{eqn:c5}) to
\begin{IEEEeqnarray*}{rCl}
 (\text{\ref{eqn:c5}})
&\overset{\text{(\ref{eqn:c1}),(\ref{eqn:c2})}}{\Leftrightarrow}&
ap_{2n}p_{2n+1}+\frac{b}{a}+
\frac{1}{p_{2n}^2+p_{2n+1}^2}\times\\
&&\times\bigg(\frac{1}{a}\left(p_{2n}(p_{2n+3}-p_{2n-1})+p_{2n+1}(p_{2n-2}-p_{2n+2})\right)+\\
&&+q_{2n-1}p_{2n-2}p_{2n}+q_{2n+1}p_{2n+1}p_{2n+3}\bigg)\in\ell^2\\
&\overset{\text{(\ref{eqn:C2})}}{\Leftrightarrow}&
ap_{2n}p_{2n+1}+\frac{b}{a}+\frac{q_{2n-1}p_{2n}^2+q_{2n+1}p_{2n+1}^2}{p_{2n}^2+p_{2n+1}^2}\in\ell^2\\
&\overset{\text{(\ref{eqn:C3}),(\ref{eqn:C2})}}{\Leftrightarrow}&
0\in\ell^2,
\end{IEEEeqnarray*}
so this condition turns out to be obsolete.

Finally, we draw our attention to (\ref{eqn:c2}). By Theorem~\ref{thm:freeparameters} we have that
the denominator of $\rho_{2n}$ is uniformly smaller than zero and hence

 \begin{IEEEeqnarray*}{rCl}
  (\text{\ref{eqn:c2}})
 &\overset{\text{(\ref{eqn:c1}),(\ref{eqn:C2})}}{\Leftrightarrow}&
\frac{1}{a^2}+q_{2n-1}p_{2n}p_{2n+1}-\frac{1}{a}p_{2n}^2-\frac{1}{a}p_{2n+1}^2\in\ell^2\\
&\overset{\text{(\ref{eqn:C3}),(\ref{eqn:C2})}}{\Leftrightarrow}&
p_{2n}^2+p_{2n+1}^2+a^2p_{2n}^2p_{2n+1}^2+bp_{2n}p_{2n+1}-\frac{1}{a}\in\ell^2.
\end{IEEEeqnarray*}

\end{proof}



==> 5.kscondition.tex <==
\begin{defdistance}
 \label{def:distance}
For two sequences $a=\{a_n\}_{n\in\mathbb N_0}$ and $a^\prime=\{a^\prime_n\}_{n\in\mathbb N_0}$ we define their distance as
\begin{equation*}
 \dist^2(a,a^\prime)=\sum_{n=0}^\infty 2^{-n}\left(a_n-a^\prime_n\right)^2.
\end{equation*}
Let us denote by $\mathcal C$ the set of constant sequences, i.e., $a^\prime\in\mathcal C$ if $a^\prime_n=a^\prime_0$ for all $n\geq0$.
We define
\begin{equation*}
 \dist^2(a,\mathcal C)=\inf_{a^\prime\in\mathcal C}\dist^2(a,a^\prime).
\end{equation*}
\end{defdistance}
We have the following lemma:
\begin{lemmakscond}
 \label{lemma:kscond}
Let $a=\{a_n\}_{n\in\mathbb N_0}$ and $b=\{b_n\}_{n\in\mathbb N_0}$ be two real one-sided sequences.
 If 
\begin{equation}
\label{eqn:kscondreq}
\sum_{k\geq0}\dist^2\left((S_+^*)^ka,\mathcal C\right)<\infty \qquad \text{and} \qquad\sum_{k\geq0}\dist^2\left((S^*_+)^ka,\mathcal C\right)<\infty,
\end{equation}
then
\begin{equation}
\label{eqn:kscondsum}
 \sum_{k\geq0}\dist^2\left((S_+^*)^k(a+b),\mathcal C\right)<\infty.
\end{equation}
In case that, additionally, $a,b\in\ell^\infty_+$ we have that
\begin{equation}
\label{eqn:kscondprod}
 \sum_{k\geq0}\dist^2\left((S_+^*)^k(a\cdot b),\mathcal C\right)<\infty.
\end{equation}
Moreover, if $a_n=\sum_{k=0}^n\alpha_j$ and $\alpha\in\ell^2_+$ then
\begin{equation}
 \label{eqn:kscondltwo}
\sum_{k\geq0}\dist^2\left((S_+^*)^ka,\mathcal C\right)<\infty.
\end{equation}
\end{lemmakscond}
\begin{proof}
 We assume (\ref{eqn:kscondreq}). Let $c^{(k)}=(c_k,c_k,\ldots)\in\mathcal C$ and $d^{(k)}=(d_k,d_k,\ldots)\in\mathcal C$ such that
\begin{IEEEeqnarray*}{rCl}
 \dist^2\left((S_+^*)^ka,c^{(k)}\right) &\leq& \dist^2\left((S_+^*)^ka,\mathcal C\right)+2^{-k},\\
\dist^2\left((S_+^*)^kb,d^{(k)}\right) &\leq& \dist^2\left((S_+^*)^kb,\mathcal C\right)+2^{-k}.
\end{IEEEeqnarray*}
It follows that
\begin{IEEEeqnarray*}{rCl}
 \dist^2\left((S^*_+)^k(a+b),\mathcal{C})\right)
&\leq& \dist^2\left((S_+^*)^k(a+b),c^{(k)}+d^{(k)}\right)\\
& = &
\sum_{n\geq0}2^{-n}\left(a_{n+k}+b_{n+k}-c_k-d_k\right)^2\\
&\leq &
\sum_{n\geq0}2^{-n+1}\left((a_{n+k}-c_k)^2+(b_{n+k}-d_k)^2\right)\\
&=& 2\dist^2\left((S_+^*)^k a,c^{(k)}\right)+2\dist^2\left((S_+^*)^k b,d^{(k)}\right)\\
&\leq&2 \left(2^{-k+1}+\dist^2\left((S_+^*)^k a,\mathcal C\right)+\dist^2\left((S_+^*)^kb,\mathcal C\right)\right),
\end{IEEEeqnarray*}
which proves (\ref{eqn:kscondsum}).

Let additionally $b\in\ell^\infty_+$. Then $d=\{d_1,d_2,\ldots\}\in\ell^\infty_+$ and
\begin{IEEEeqnarray*}{l}
 \dist^2\left((S_+^*)^k(a\cdot b),\mathcal C\right)
\leq
\dist^2\left((S_+^*)^k(a\cdot b),c^{(k)}\cdot d^{(k)}\right)\\
\qquad=
\sum_{n\geq0}2^{-n}\left(a_{n+k}(b_{n+k}-d_k)+d_k(a_{n+k}-c_{k})\right)^2\\
\qquad\leq
\sum_{n\geq0}2^{-n+1}\left(
\|a\|_{\infty}^2\left(b_{n+k}-d_k\right)^2+\|d\|_{\infty}^2\left(a_{n+k}-c_k\right)^2\right)\\
\qquad=
2\|d\|^2_{\infty}\dist^2\left((S_+^*)^ka,c^{(k)}\right)+\|a\|_{\infty}^2\dist^2\left((S_+^*)^kb,d^{(k)}\right)\\
\qquad\leq
2\|d\|^2_{\infty}\left(\dist^2\left((S_+^*)^ka,c^{(k)}\right)+2^{-k}\right)+
2\|a\|^2_{\infty}\left(\dist^2\left((S_+^*)^kb,d^{(k)}\right)+2^{-k}\right)
\end{IEEEeqnarray*}
and hence (\ref{eqn:kscondprod}) follows.

Finally, let $a_n=\sum_{j=0}^n\alpha_j$ and $\alpha\in\ell^2_+$. In order to estimate the infimum we choose $(a_k,a_k,\ldots)$ as a constant sequence for 
each $k$ and thus obtain
\begin{IEEEeqnarray*}{rCl}
 \sum_{k\geq0} \dist^2\left(\left(S^*_+\right)^k a,C\right)
&\leq&
\sum_{k\geq0}\sum_{n\geq0}2^{-n}\left(\sum_{j=1}^n \alpha_{j+k}\right)^2
\leq \sum_{n\geq0}2^{-n}n\sum_{j=1}^n\sum_{k\geq0}\alpha_{j+k}^2\\
&\leq& \sum_{n\geq0}2^{-n}n^2\sum_{k\geq0}\alpha_k^2<\infty.
\end{IEEEeqnarray*}
\end{proof}

\begin{defdistancesmp}
 Let $\{p_n,q_n,r_n\}_{n\geq0}$ (resp. $\{p_n^{\prime},q_n^{\prime},r_n^{\prime}\}_{n\geq0}$) be a set of sequences defining 
a one-sided matrix $A_+$ (resp. $A_+^{\prime}$). Then we define their distance as
\begin{equation*}
 \dist^2\left(A_+,A_+^{\prime}\right)
=
\dist^2(p_n,p_n^{\prime})+\dist^2(q_n,q_n^{\prime})+\dist^2(r_n,r_n^{\prime}).
\end{equation*}
Furthermore, for a subset $\mathcal S$ of the SMP class we set
\begin{equation*}
 \dist^2(A_+,\mathcal S) = \inf_{A^{\prime}\in\mathcal S} \dist^2(A_+,A_+^{\prime}).
\end{equation*}

\end{defdistancesmp}

Considering the above lemma as well as Theorem~\ref{thm:freeparameters} and Lemma~\ref{lemma:ks} we have the following
theorem.
\begin{thmkscond}
 \label{thm:kscond}
Let $A\in\ks_{\smp}(E)$. Then
\begin{equation*}
 \sum_{k=-1}^\infty\dist^2\left(\left(S^{-2k}AS^{2k}\right)_+, A_0(E)\right)<\infty.
\end{equation*}
\end{thmkscond}


\begin{comment}
\begin{proof}
The claim immediately follows for $\{r_n\}$, since $r_{2n}=0$ and, due to (\ref{eqn:C1}) from Lemma~\ref{lemma:ks}, 
$r_{2n+1}-a^{-1}\in\ell^2_+$. For $\{p_n\}$ we choose $p_k$ for each $k$ as a constant sequence and observe that, by (\ref{eqn:C2}),
we have, for instance,
\begin{equation*}
 p_{2n}=\alpha_{2n}+\alpha_{2n-2}+\ldots+p_0
\end{equation*}
 for some $\alpha_{2n}\in\ell^2_+$. By (\ref{eqn:kscondltwo}) we see that the claim holds true for $\{p_n\}$.

From Theorem~\ref{thm:freeparameters} we already know that
\begin{equation*}
 q_{2n}=\frac{p_{2n}p_{2n+1}}{r_{2n+1}}.
\end{equation*}
Hence, with a view to (\ref{eqn:C1}), we choose as our constant  sequence (w.r.t. $n$) $ap_{2k}p_{2k+1}$. Furthermore, note that
\begin{IEEEeqnarray*}{rcl}
 q_{2n}-ap_{2k}p_{2k+1}&=&\left(\frac{1}{r_{2(n+k)+1}}-a\right)p_{2(n+k)}p_{2(n+k)+1}
-a\Bigg(p_{2k}\left(p_{2(k+n)+1}-p_{2k+1}\right)\\
&&+p_{2k+1}\left(p_{2(k+n)}-p_{2k}\right)
+\left(p_{2(k+n)}-p_{2k}\right)\left(p_{2(k+n)+1}-p_{2k+1}\right)\Bigg).
\end{IEEEeqnarray*}
Since $\{r_{2n+1}\}$ is uniformly greater than zero and $\{p_n\}$ is uniformly bounded the result now follows from (\ref{eqn:C1})
together with Theorem~\ref{thm:kscond} and the fact that $p_n$ can be approximated by $p_k$.

Finally, we have that
\begin{IEEEeqnarray*}{l}
 q_{2(n+k)+1}+\frac{b}{a}+ap_{2k}p_{2k+1}=\\
\quad=q_{2(n+k)+1}+\frac{b}{a}+ap_{2(n+k)+1}p_{2(n+k)}+a\Bigg(p_{2(n+k)+1}\left(p_{2k}-p_{2(n+k)}\right)\\
\quad+p_{2(n+k)}\left(p_{2k+1}-p_{2(n+k)+1}\right)+\left(p_{2k}-p_{2(n+k)}\right)\left(p_{2k+1}-p_{2(n+k)+1}\right)\Bigg)
\end{IEEEeqnarray*}
and by (\ref{eqn:C3}) and similar reasons as we had above we obtain the desired result.
\end{proof}
\end{comment}


==> 6.parametrization.theorem.tex <==
We set
\begin{equation*}
 p_{2n}=R_n\cos\phi_n,\qquad p_{2n+1}= R_n\sin\phi_n
\end{equation*}
and obtain the following result.
\begin{thmks}
 \label{thm:ks}
$A\in\ks_{\smp}(E)$ if and only if there exist sequences $\{\alpha_n\}$, $\{\beta_n\}$, $\{\gamma_n\}$, $\{\delta_n\}\in\ell^2$ such that
\begin{align}
  \tag{KS1}
 \phi_n&=\phi_0+\sum_{k=1}^n \alpha_n,	 \label{eqn:KS1}\\
 \tag{KS2a}
 p_{2n}&=\left(R(\phi_n)+\beta_n\right)\cos\phi_n,	 \label{eqn:KS2a}\\
 \tag{KS2b} 
 p_{2n+1}&=\left(R(\phi_n)+\beta_n\right)\sin\phi_n,	 \label{eqn:KS2b}\\
\tag{KS3}
q_{2n+1}&= -\frac{1}{2}R^2(\phi_n)\sin(2\phi_n)-\frac{b}{a}+\gamma_n,	 \label{eqn:KS3}\\
\tag{KS4}
r_{2n+1}&=\frac{1}{a}+\delta_n,	\label{eqn:KS4}
\end{align}
where
\begin{equation*}
 R^2(\phi)\deq\frac{1}{a} \frac{4}{\sqrt{(2+b\sin(2\phi))^2+4a\sin^2(2\phi)}+2+b\sin(2\phi)}.
\end{equation*}
\end{thmks}

\begin{proof}
 Obviously, (\ref{eqn:KS4}) is just a reformulation of (\ref{eqn:C1}).
Let us continue with (\ref{eqn:C4}). There exists a sequence $\{\beta^\prime_n\}\in\ell^2$ such that
\begin{equation*}
 R_n^2+a^2R_n^4\frac{\sin(2\phi_n)}{4}+bR_n^2\frac{\sin(2\phi_n)}{2}-\frac{1}{a}=\beta_n^\prime.
\end{equation*}
We solve this equation for $R_n^2$ and obtain
\begin{equation*}
 R_n^2=\frac{-(2+b\sin(2\phi_n))\pm\sqrt{(2+b\sin(2\phi_n))^2+4a(1+a\beta_n^\prime)\sin^2(2\phi_n)}}{a^2\sin^2(2\phi_n)}.
\end{equation*}
Note that $R_n^2$ has to be non-negative. Hence, we have to choose the solution with the plus sign. Further simplifications yield 
\begin{equation*}
 R_n^2=\frac{1}{a}\frac{4(1+a\beta_n^\prime)}{\sqrt{(2+b\sin(2\phi_n))^2+4a(1+a\beta^\prime_n)\sin^2(2\phi_n)}+2+b\sin(2\phi_n)}.
\end{equation*}
% NEW
Moreover, the function 
\begin{equation*}
 g(x)\deq\sqrt{\left(2+bx\right)^2+4 ax^2}+2+bx,\quad x\in\mathbb R
\end{equation*}
attains its minimum at 
\begin{equation*}
 x_0=-\frac{4b}{4a+b^2}\quad\text{and}\quad g(x_0)=\frac{16a}{4a+b^2}>0.
\end{equation*}
\begin{comment}
\begin{equation*}
 \sqrt{\left(\frac{2+b\sin(2\phi)}{2a}\right)^2+\frac{\sin^2(2\phi)}{a}}+\frac{2+b\sin(2\phi)}{2a}\geq-a_1>0
\end{equation*}
\end{comment}

Hence, $R_n^2-R^2(\phi_n)\in\ell^2$.
Thus, we immediately obtain (\ref{eqn:KS2a}), (\ref{eqn:KS2b}) and (\ref{eqn:KS3}).
 
Now, consider (\ref{eqn:C2}), i.e.
\begin{IEEEeqnarray*}{c}
 R_n\cos\phi_n-R_{n-1}\cos\phi_{n-1}\in\ell^2\quad\text{and}\quad R_n\sin\phi_n-R_{n-1}\sin\phi_{n-1}\in\ell^2
\end{IEEEeqnarray*}
Rewriting the cosines and sines by means of the exponential function and adding these two conditions gives
\begin{equation*}
 (\ref{eqn:C2})\Longleftrightarrow e^{\im\phi_n}-e^{\im\phi_{n-1}}\in\ell^2
\Longleftrightarrow\sin\left(\frac{\phi_n-\phi_{n-1}}{2}\right)\in\ell^2
\Longleftrightarrow\phi_n-\phi_{n-1}\in\ell^2,
\end{equation*}
which is exactly (\ref{eqn:KS1}).
\end{proof}
% NEW
\begin{reminnerouttercircle}
 \label{rem:innerouttercircle}
Let $g$ be defined as in the above proof. For $x\in[-1,1]$ we set
\begin{equation*}
 f(x)\deq \frac{1}{2a} g(x)=\sqrt{\left(\frac{2+bx}{2a}\right)^2+\frac{x^2}{a}}+\frac{2+bx}{2a}.
\end{equation*}
Note that, for $b<0$, we have that $f(x)\leq f(-1)=a_0$ and, for $b>0$, $f(x)\leq f(1)=-b_0$ (for $b=0$ these two values coincide).
Therefore, the radius of the incircle of the isospectral curve is given by
\begin{equation*}
 r_{in}=\sqrt{\frac{2}{a^2 \max\{a_0,-b_0\}} }.
\end{equation*}
\begin{comment}
For the determination of the excircle we can use the minimum $x_0$ of the function $g$ from the above proof. However, 
$x_0\in[-1,1]$ is not automatically fulfilled. In the case where $x_0>1$ one can show that $f(x_0)\geq-b_0$ and if $x_0<-1$ we have that $f(x_0)\geq a_0$.
Since these values are attained by $f$ the radius of the excircle is given by
\begin{equation*}
 r_{ex}= \frac{\sqrt{2}}{a} \left\{
\begin{array}{clr}
\sqrt{a_0}	& \text{if } &	x_0<-1,\\
\sqrt{\frac{4a+b^2}{8}} & \text{if }& -1\leq x_0\leq 1,\\
\sqrt{-b_0}	&	\text{if }&  x_0>1.
\end{array}
\right.
\end{equation*}
\end{comment}

\end{reminnerouttercircle}

Figure 3 shows a plot of the isospectral curve $(R(\phi)\cos(\phi),R(\phi)\sin(\phi))$ in the $(p_0,p_1)$-plane.

\begin{figure}[!hbtp]
\phantomsection
\label{fig:r}
 \centering
  \includegraphics[width=0.5\textwidth]{r.jpg}
 \caption[The isospectral curve in the $(p_0,p_1)$-plane]{The isospectral curve in the $(p_0,p_1)$-plane for $a=2.5$ and $b=-3$.}
\end{figure}

==> bib.tex <==
\begin{thebibliography}{99}	
\bibitem{schur} L. Baratchart, S.~Kupin, V.~Lunot, M. Olivi, \emph{Multipoint Schur algorithm and orthogonal rational functions,
I: Convergence properties.}
  Journal D'Analyse Mathématique 114 (2011),  207-253.

\bibitem{jreview} J. S. Christiansen, B.~Simon, M.~Zinchenko, \emph{Finite gap Jacobi matrices: A review.}
   arXiv:1301.5073v2 [math.SP] 

\bibitem{refjreview} D. Damanik, R.~Killip, B. Simon, \emph{Pertubations of orthogonal polynomials with periodic recursion coefficients.}
  Annals of Math. 171 (2010), 1931-2010.

\bibitem{2003}R. Killip, B. Simon, \emph{Sum rules for Jacobi matrices and their applications to spectral theory. }
Annals of Math. (2)  158  (2003),  no. 1, 253-321.

\bibitem{smp} I. Moale, P.~Yuditskii, \emph{Parametrization of spectral surfaces of a class of periodic 5-diagonal matrices.}
   	arXiv:1112.3219 [math.SP]

\bibitem{shmp} O.~Nj{\aa}stad, \emph{Solutions of the strong Hamburger moment problem.} 
  J. Math. Anal. Appl. 197 (1996), 227-248.

 \bibitem{2005v1}B. Simon,
\emph{Orthogonal polynomials on the unit circle. Part 1.} Classical theory, 
American Mathematical Society Colloquium Publications, 54, Part 1. American Mathematical Society, Providence, RI, 2005. xxvi+466 pp. 


\bibitem{2005v2}B. Simon, 
\emph{Orthogonal polynomials on the unit circle.  Part 2.} Spectral theory, American Mathematical Society Colloquium Publications, 54,
 Part 2. American Mathematical Society, Providence, RI, 2005. pp. i–xxii and 467–1044. 


\end{thebibliography}

==> intro.tex <==
Jacobi matrices probably are the most classical object in spectral theory, while CMV matrices are a comparably fresh one \cite{2005v1,2005v2}, 
although they
are related to a very classical topic, namely to orhtogonal polynomials on the unit circle (in the same way as Jacobi matrices are related
to orhogonal polynomials on the real axis). We will discuss the third member of this family. Our matrices are generated by the 
orthonormal systems of functions related to the so-called \emph{Strong Moment Problem} (see, for instance, \cite{shmp} and references
therein). 
For this reason we call them \emph{SMP matrices}.


In their breakthrough paper \cite{2003} R.~Killip and B.~Simon completely described spectral properties of Jacobi matrices $J_+$
which are Hilbert-Schmidt-class pertubations of matrices with constant coefficients. That is, let
\begin{equation*}
 J_+e_n=a_{n}e_{n-1}+b_ne_n+a_{n+1}e_{n+1},\quad a_{0}=0,
\end{equation*}
where $\{e_n\}_{n\geq0}$ is the standard basis in $\ell^2_+$.
Then
\begin{equation*}
 \sum_n\left((a_n-1)^2+b_n^2\right)<\infty
\end{equation*}
if and only if the spectrum of $J_+$ is the union of the interval $[-2,2]$ and an at most countable system of points $X=\{x_k\}$
accumulating to the ends of the interval only and 
\begin{equation*}
 \int^{2}_{-2}|\log\sigma^\prime(x)|\sqrt{4-x^2}\ud x+\sum_{x_k\in X}\sqrt{x_k^2-4}^3<\infty,
\end{equation*}
where $\sigma$ denotes the spectral measure of $J_+$.

In \cite{refjreview} this result was generalized to the case of pertubations of (non-degenerated) \emph{periodic} matrices. The 
main idea behind this is a reduction of the initial problem to the problem related to 
pertubations of Jacobi matrices with \emph{constant} \emph{matrix-block} coefficients.

Recall that the spectrum $E$ of a $p$-periodic Jacobi matrix $J_0$ is of the form $E=T^{-1}\left([-2,2]\right)$, where $T(z)$ is
a polynomial. In the non-degenerated case $T$ is of degree $p$ and $E$ consists of exactly $p$ intervals. Let $J_0(E)$ be
the collection of all periodic matrices with given spectrum $E$. Then the so-called Magic Formula holds true: 
\begin{equation}
 \label{eqn:magicformula}
T(J_0)=S^{p}+S^{-p}
\end{equation}
for every $J_0\in J_0(E)$. Now, the Killip-Simon-class $\ks_J(E)$ can be fully characterized as the collection of $J$'s for 
which $T(J)-(S^{p}+S^{-p})$ belongs to the Hilbert-Schmidt-class. Thus, $T(J)$ is a block-Jacobi matrix whose block-coefficients
are close to the $p\times p$ block-matrix $S^{p}+S^{-p}$ with constant coefficients. After that, the class $\ks_J(E)$ was completely characterized
in spectral terms as well as w.r.t. coefficient sequences (by means of approaching of the shifts of $J$ to the isospectral set $J_0(E)$).

In \cite{jreview}  the following problem was posed: ``Is there an extention of the Damanik-Killip-Simon theorem to the general 
$E$ case?''. Note that, in the two-interval case, the Damanik-Killip-Simon method can only be used if $E$ is the union of two intervals
of \emph{equal} length. We are able to study the case of two \emph{arbitrary} intervals, but for SMP matrices.
We propose a magic formula for
periodic SMP matrices $A_0$ with the given spectrum $E$, i.e., (compare to (\ref{eqn:magicformula}))
\begin{equation*}
 V(A_0)=S^2+S^{-2},
\end{equation*}
where $V(z)$ denotes a special rational function (see Theorem~\ref{thm:isospectral} for more details).
Subsequently, we will define the Killip-Simon-class $\ks_{\smp}(E)$ for SMP matrices $A$ by $V(A)-(S^2+S^{-2})$ being a Hilbert-Schmidt operator.
Thus, the theorem on pertubations of Jacobi matrices with block-matrix coefficients can be used perfectly well in our case.
In particular, we can get spectral properties of $A$ in the same way as in \cite{refjreview}.
As the main result of this paper we give a parametric description of the coefficients of the elements from $\ks_{\smp}(E)$, see  Theorem~\ref{thm:ks}.

Furthermore, we present a similar explicit parametrization for Jacobi matrices with their essential spectrum on two symmetric intervals.
We begin by dealing with this as an introductory problem. The structure of the paper is given in the table of contents.
